Towards Dynamic 3D Reconstruction of Hand-Instrument Interaction in Ophthalmic Surgery

Accurate 3D reconstruction of hands and instruments is critical for vision-based analysis of ophthalmic microsurgery, yet progress has been hampered by the lack of realistic, large-scale datasets and reliable annotation tools. In this work, we introduce OphNet-3D, the first extensive RGB-D dynamic 3D reconstruction dataset for ophthalmic surgery, comprising 41 sequences from 40 surgeons and totaling 7.1 million frames, with fine-grained annotations of 12 surgical phases, 10 instrument categories, dense MANO hand meshes, and full 6-DoF instrument poses. To scalably produce high-fidelity labels, we design a multi-stage automatic annotation pipeline that integrates multi-view data observation, data-driven motion prior with cross-view geometric consistency and biomechanical constraints, along with a combination of collision-aware interaction constraints for instrument interactions. Building upon OphNet-3D, we establish two challenging benchmarks-bimanual hand pose estimation and hand-instrument interaction reconstruction-and propose two dedicated architectures: H-Net for dual-hand mesh recovery and OH-Net for joint reconstruction of two-hand-two-instrument interactions. These models leverage a novel spatial reasoning module with weak-perspective camera modeling and collision-aware center-based representation. Both architectures outperform existing methods by substantial margins, achieving improvements of over 2mm in Mean Per Joint Position Error (MPJPE) and up to 23% in ADD-S metrics for hand and instrument reconstruction, respectively.

==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related}

Surgical vision research has recently evolved beyond traditional tasks~\cite{nwoye2021rendezvous, hu2024ophnet, grammatikopoulou2021cadis} toward 3D perception, including scene reconstruction~\cite{zha2023endosurf, cotsoglou2024dynamic}, depth estimation~\cite{cui2024surgical, yang2024self}, and navigation~\cite{qiu2020endoscope, yang2024slam}. Despite advances in datasets like AVOS~\cite{goodman2024analyzing} and MM-OR~\cite{ozsoy2025mm}, most systems remain limited to passive monitoring rather than real-time surgical assistance. Meanwhile, 3D hand reconstruction has progressed from general benchmarks~\cite{zimmermann2019freihand, moon2020interhand2} to synthetic medical datasets~\cite{wang2023pov, birlo2024hup}, though lacking clinical realism. Monocular approaches have evolved from single-hand models~\cite{dong2024hamba, pavlakos2024reconstructing} to two-hand systems~\cite{zhang2021interacting, lin20244dhands} and hand-object interactions~\cite{wu2024reconstructing, ye2023diffusion}, using template-based methods~\cite{garcia2018first, hampali2020honnotate} and geometric constraints~\cite{brahmbhatt2020contactpose, zhang2020perceiving}. Our work bridges the clinical gap with a targeted 3D perception framework for ophthalmic microsurgery using real RGB-D data capturing fine-grained, two-hand, multi-instrument interactions. See Tab.~\ref{tab:comp_general} and ~\ref{sec:related_appendix} for detailed comparisons.

% Recent surgical vision research has expanded beyond traditional tasks such as phase recognition~\cite{nwoye2021rendezvous, hu2024ophnet, hu2023nurvid, hu2024ophclip} and anatomical segmentation~\cite{borgli2020hyperkvasir, grammatikopoulou2021cadis} to address 3D perception challenges in open surgical environments, including scene reconstruction~\cite{zha2023endosurf, cotsoglou2024dynamic, hayoz2024online, chen2025endoperfecthybridnerfstereovision}, depth estimation~\cite{cui2024surgical, yang2024self, tian2024endoomni, liu2019dense}, and navigation~\cite{qiu2020endoscope, bartholomew2024surgical, yang2024slam, manni2024bodyslam}. While datasets like AVOS~\cite{goodman2024analyzing} and MM-OR~\cite{ozsoy2025mm} have advanced multimodal capabilities, most systems remain limited to passive monitoring or offline analysis rather than real-time surgical assistance. Concurrently, 3D hand reconstruction has progressed through general benchmarks like FreiHAND~\cite{zimmermann2019freihand} and InterHand2.6M~\cite{moon2020interhand2}, with medical extensions such as POV-Surgery~\cite{wang2023pov} and HUP-3D~\cite{birlo2024hup}, though these synthetic datasets lack clinical realism. Monocular reconstruction approaches have evolved from single-hand models~\cite{dong2024hamba, li2024hhmr, pavlakos2024reconstructing, kim2023sampling, yu2023acr} to two-hand systems~\cite{zhang2021interacting, yu2023acr, lin20244dhands, ren2023decoupled} and hand-object interactions~\cite{wu2024reconstructing, prakash20243d, huang2022hhor, ye2023diffusion}, employing techniques ranging from template-based methods~\cite{garcia2018first, hamer2010object, hampali2020honnotate} to joint reasoning via feature fusion~\cite{chen2021joint, gkioxari2018detecting, liu2021semi, shan2020understanding, tekin2019h+} and geometric constraints~\cite{brahmbhatt2020contactpose, cao2021reconstructing, corona2020ganhand, grady2021contactopt, zhang2020perceiving}. Our work addresses the clinical gap by developing a targeted 3D perception framework for ophthalmic microsurgery with real RGB-D data capturing fine-grained, two-hand, multi-instrument interactions. For a comprehensive comparison of datasets and methods, please refer to Tab.~\ref{tab:comp_general} and ~\ref{sec:related_appendix}.


% \noindent \textbf{Surgical 3D Perception.} 
% Beyond conventional tasks in surgical assistance such as phase recognition~\cite{nwoye2021rendezvous, hu2024ophnet, hu2023nurvid, hu2024ophclip}, anatomical segmentation~\cite{borgli2020hyperkvasir, grammatikopoulou2021cadis} and instrument detection~\cite{hu2024ophclip, nwoye2021rendezvous}, recent efforts have increasingly focused on 3D perception for open surgical environments, addressing challenges in scene reconstruction~\cite{zha2023endosurf, cotsoglou2024dynamic, hayoz2024online, chen2025endoperfecthybridnerfstereovision}, depth estimation~\cite{cui2024surgical, yang2024self, tian2024endoomni, liu2019dense}, navigation~\cite{qiu2020endoscope, bartholomew2024surgical, yang2024slam, manni2024bodyslam}, and skill assessment~\cite{liu2021towards, goodman2024analyzing}. A growing body of work leverages multi-view camera arrays, RGB-D sensors, and IMUs to reconstruct dense surgical scenes with both static anatomical structures and dynamic hand-tool interactions. Goodman et al.~\cite{goodman2024analyzing} proposed AVOS, a large-scale annotated video dataset of open surgeries, and developed a multitask model to extract procedural signatures and quantify surgeon skill from real-world surgical videos. MM-OR~\cite{ozsoy2025mm} introduces a comprehensive multimodal operating room dataset featuring RGB-D, audio, speech transcripts, and robotic logs, annotated with panoptic segmentation and semantic scene graphs. While these systems demonstrate technical progress on specific tasks and in multimodal fusion capabilities, their clinical impact remains limited, with most systems designed primarily for passive action recognition or offline documentation. Few are optimized for real-time use or tailored to support specific training objectives in microsurgical procedures. In this work, we address this gap by developing a clinically-oriented 3D perception framework for ophthalmic microsurgery, integrating task-specific data, model design, and system-level considerations for real-world deployment.

% \noindent \textbf{3D Hand Dataset.} 
% Recent 3D hand reconstruction datasets have driven progress in hand pose, object pose, and interaction reconstruction (see Tab.~\ref{tab:comp_general}). General benchmarks such as FreiHAND~\cite{zimmermann2019freihand} and InterHand2.6M~\cite{moon2020interhand2} provide multi-view real RGB images for reliable 3D pose recovery. ContactPose~\cite{brahmbhatt2020contactpose} further leverages RGB-D to capture detailed contact patterns. Banerjee et~al. present HOT3D~\cite{banerjee2024hot3d}, a large-scale egocentric, multi-view hand--object interaction (HOI) dataset comprising $\approx$1.5\,M synchronized frames captured with head-mounted Aria and Quest~3 cameras across 19 participants manipulating 33 objects; each frame is paired with mocap-grade 3D hand and object poses. Medical datasets extend these ideas to surgery. Hein et al.~\cite{hein2021towards} released a synthetic surgical RGB set with limited views and simple actions. POV-Surgery~\cite{wang2023pov} and HUP-3D~\cite{birlo2024hup} enrich viewpoint count and interaction diversity, yet their synthetic origin still curbs realism. Ophthalmic surgery, notably cataract removal, follows fixed workflows but requires both hands to manipulate several tools in a confined field—for instance, holding an iris retractor while guiding capsulorhexis forceps. These dense, dual-hand motions strain current reconstruction methods. OphNet-3D addresses this gap with a real RGB-D clinical dataset that records fine-grained, two-hand, multi-instrument interactions during live ophthalmic operations.

% \noindent \textbf{Monocular 3D Hand Mesh Reconstruction.} 
% Compared with multi‑view approaches, monocular reconstruction is more practical in clinical theatres: a single, non‑contact RGB camera minimises equipment, preserves sterility, and avoids obstructing the surgeon’s workspace. Research has progressed from single‑hand models~\cite{dong2024hamba, li2024hhmr, pavlakos2024reconstructing, kim2023sampling, yu2023acr} to two‑hand systems~\cite{zhang2021interacting, yu2023acr, lin20244dhands, ren2023decoupled} and, most recently, HOI reconstruction~\cite{wu2024reconstructing, prakash20243d, huang2022hhor, ye2023diffusion}. Monocular HOI remains difficult because occlusion is severe and annotated data are scarce. Many studies therefore assume known instance‑specific templates~\cite{garcia2018first, hamer2010object, hampali2020honnotate}; with the template in place, object recovery reduces to 6D pose estimation and joint hand–object pose inference. Joint reasoning is implemented via implicit feature fusion~\cite{chen2021joint, gkioxari2018detecting, liu2021semi, shan2020understanding, tekin2019h+}, explicit geometric constraints such as contact or collision~\cite{brahmbhatt2020contactpose, cao2021reconstructing, corona2020ganhand, grady2021contactopt, zhang2020perceiving}, or physics‑based consistency~\cite{pham2017hand, tzionas2016capturing}. To lift the template assumption, newer work directly predicts object shape—either as explicit genus‑0 meshes~\cite{hasson2019learning} or via a joint hand–object implicit field~\cite{karunratanakul2020grasping}. Conditional reconstruction strategies further exploit hand joint cues to refine object geometry~\cite{ye2022s}.

